CELEST: Federated Learning for Globally Coordinated Threat Detection

The cyber-threat landscape has evolved tremendously in recent years, with new threat variants emerging daily, and large-scale coordinated campaigns becoming more prevalent. In this study, we propose CELEST (CollaborativE LEarning for Scalable Threat detection, a federated machine learning framework for global threat detection over HTTP, which is one of the most commonly used protocols for malware dissemination and communication. CELEST leverages federated learning in order to collaboratively train a global model across multiple clients who keep their data locally, thus providing increased privacy and confidentiality assurances. Through a novel active learning component integrated with the federated learning technique, our system continuously discovers and learns the behavior of new, evolving, and globally-coordinated cyber threats. We show that CELEST is able to expose attacks that are largely invisible to individual organizations. For instance, in one challenging attack scenario with data exfiltration malware, the global model achieves a three-fold increase in Precision-Recall AUC compared to the local model. We also design a poisoning detection and mitigation method, DTrust, specifically designed for federated learning in the collaborative threat detection domain. DTrust successfully detects poisoning clients using the feedback from participating clients to investigate and remove them from the training process. We deploy CELEST on two university networks and show that it is able to detect the malicious HTTP communication with high precision and low false positive rates. Furthermore, during its deployment, CELEST detected a set of previously unknown 42 malicious URLs and 20 malicious domains in one day, which were confirmed to be malicious by VirusTotal.

==> background.tex <==
\subsection{Background on Federated Learning and NLP}
\label{sec:background}

\input{background/FL}
\input{background/NPL}








\begin{comment}

\subsection{Problem Definition and Threat Model}
In this section, we discuss the problem definition and threat model, and provide background on word embeddings and federated learning to train global models.

\subsubsection{HTTP-based Malware Activity}

Hyper-Text-Transfer-Protocol (HTTP) is one of the most widely used communication protocols across the internet. Adversaries use HTTP to blend in with the benign traffic to avoid detection during execution of different malicious activities. These activities are known involve command and control (C2) communication~\cite{httpC22021, sood2014empirical}, data exfiltration~\cite{dataExfilt2020}, vulnerability exploitation~\cite{httpmirai2019} and covert channel communication~\cite{httpstatusmalware2020}. 
%Recent malware campaigns involve a variety of operations on different ports, and they HTTP is still one of the actively used methods observed around the world. 
% Some malware are known to utilize HTTPs instead of HTTP to encrypt the malicious activity, but 
Prior work proposed a variety of intrusion detection methods based on malicious URL/host detection~\cite{mamun2016detecting, mcgahagan2019comprehensive}, HTTP-application fingerprinting~\cite{perdisci2010behavioral, bortolameotti2017decanter, bortolameotti2020headprint}  to help mitigate this threat. While malicious URL detection is shown to be successful in mitigating certain attacks (e.g., phishing), an HTTP-head based detection method is stronger as it can address a variety of attack surfaces used by different malware families. These methods avoid deep inspection and rely on HTTP headers 

%(which improves scalability and computation cost) and independent of the payload which could be obfuscated.

Existing defenses can detect malicious HTTP traffic to some extent, either by classification or anomaly detection based methods, especially against known attack behaviors. Nevertheless, adversaries always try to find more novel methods to evade the existing defenses. Therefore, this is still an active threat facing networks and enterprises globally. As many local networks and enterprises face similar threat, threat intelligence help organizations improve their local intrusion detection systems. There are a few challenges with collaborating for intrusion detection. The process need to be automated, scalable to support a number of large networks, preserve the privacy of sensitive data, and the detection models should support processing at real-time, and minimize low false positives. Collaborative machine learning training addresses these challenges with the recent advances in federated learning~\cite{mcmahan2017communication}. In this work, we propose a new method to detect malicious HTTP events, and utilize federated learning to further enable global defense mechanisms in a scalable way.

%- Requirements: http logs, preserve the privacy, real-time deployment, scalability, low false positives, resilient to evasion?, limited labels, data is anonymized,  

\subsubsection{Threat Model}

Hosts in the network can be infected in a variety of ways, e.g. vulnerability exploit, social-engineering, drive-by download. We consider adversaries that attack multiple networks globally. We aim to detect malicious activity in the context of incoming and outgoing http connections, as an indication of infection, vulnerability exploit, or C2 communication. In this work, we only consider HTTP-based malware activity. Although, HTTPs-based malware have been observed recently, we do not consider them in this work. TLS proxies can observe the encrypted HTTPs communication and our methods could be applied.
% there are works on detecting https communications as well, using a subset of our features, we can adapt our system for that
We assume there are correct malicious labels available for HTTP logs, and machine learning model training is safe. During federated training, we assume the communication channels are secure, and participating organizations (clients) are trusted. 

%In future, we will expand our work to consider adversarial clients. 



\subsection{Background on Federated Learning}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\textwidth]{figs/fed_diagram}
	\caption{Overview of the federated learning framework.}
	\label{figure:fed}
\end{figure*}

\begin{algorithm}[t]
	\caption{\texttt{FederatedLearning(fedAvg).}  $W$ is the model weights, $M$ is the participating clients, $n$ is the number of data points, $B$ is the local dataset, $\eta$ is the learning rate}\label{alg:fedavg}
	\begin{algorithmic}[1]
		\State Initialize $W_0$
		\Procedure{ServerExecute}{W, M}
		\For{ each round $t$ }
		\State $S_m \leftarrow $ (pick $m$ clients from $M$)
		\For{each client $k \in S_m$ \textbf{in parallel}}
		\State $W_{t+1}^k \leftarrow \text{ClientUpdate}(k, W_t)$ 
		\EndFor
		\State $w_{t+1} \leftarrow \sum_{k \in S_m} \frac{n_k}{n} w_{t+1}^k $
		\EndFor
		\EndProcedure
		
		\Procedure{ClientUpdate}{$k$, $w_t$} \Comment{Update the global model at client k}
		\State $w_{local} \leftarrow w_t$
		\For{each local epoch}
		\For{batch $b \in B_k$}
		\State $w_{local} \leftarrow w_{local} - \eta \triangledown \ell(w_{local}, b)$
		\EndFor{}
		\EndFor{}
		\State Send $w_{local}$ to the server
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


Federated Learning is a machine learning technique designed for collectively training a global model. Multiple clients participate in the training process without sending any local data. Local training updates from each client are sent to the central server, and the updates are aggregated, and distributed back to the clients. Algorithm~\ref{alg:fedavg} describes the federated averaging algorithm proposed by~\cite{mcmahan2017communication}. 

Federated learning has been used in a variety of domains (e.g. natural language processing (NLP)) with great success. In the context of threat detection, federated learning would be helpful for both the privacy of the data in the client organizations, and improving local models by taking advantage of the experiences of known previously-detected threats from the other networks.


\subsection{Background on Embedding Models}

One of the most important signals of malicious activity is the domain name, URL string, for the destination and the referer fields of the HTTP logs. It is important to represent these accurately for machine learning algorithms to learn the important signals. There are a number of different ways to represent text proposed in the NLP community.
The traditional count-based technique for extracting semantic features is based on the family of models called Bag-of-Words, which includes methods like term frequencies, TF-IDF (term frequency-inverse document frequency), N-grams, etc. 
%In the case of URLs, the string is split into component words delimited by special characters in a URL, and all the distinct words in the training set become features~\cite{blum2010, ma2009beyond, mamun2016detecting}. Given $N$ distinct features represented by words $(w_1, w_2, ..., w_N)$, each URL is encoded as a vector $v \in R^N$, where $v_i$ is 1 if the word $w_i$ is present in the URL, and 0 otherwise. 
This feature representation was shown to have several limitations such as the large feature space, resulting in possible huge sparse vector words that lead to poor models or data overfitting. Additional limitations include the inability to capture the sequence in which words appear, as well as the inability to generalize to new words that have not been seen in training, but which may appear in testing~\cite{le2018urlnet, sahoo2017,  sarkar2018, baroni-etal-2014-dont}. 

This has been the motivation of recent research to explore more sophisticated models that use deep learning strategies to capture the context of words in a vector representation called embeddings. Some well-known methods successfully used in the NPL community are Word2Vec and FastText, which are briefly described next. 
%are Word2Vec, GloVe and FastText, which are briefly described next. 
Word2Vec is an unsupervised model invented by Mikolov et al. at Google in 2013~\cite{mikolov2013word2vec, mikolov2013distributed} that uses Neural Networks to generate dense word embeddings that capture contextual and semantic similarities such that similar words will be closer in the embedded vector space. With Word2Vec, one can predict either the target word based on the context (CBOW model) or predict the context words given the target word (Skip-gram model). 
%Another unsupervised deep learning model used to obtain dense word vectors is GloVe, created by Pennington et al. at Stanford in 2014~\cite{pennington2014glove}. In GloVe, training is done on an aggregated global word-word co-occurrence matrix that tabulates how frequently words co-occur with one another in a given corpus. While Word2Vec uses local individual examples of word co-occurrence pairs, GloVe uses global aggregated co-occurrence statistics across all words in the corpus~\cite{sarkar2018}.
%The third embedding model discussed here, 
FastText, is an extension of Word2Vec proposed in 2016~\cite{bojanowski2016enriching, joulin2016tricks}. FastText treats each word as composed of character n-grams. Thus, rare words generalize better at the expense of training space and time requirements which depend on the choice of hyper-parameters controlling the minimum and maximum n-gram sizes. 

%In parallel with these efforts from the NPL community, a few recent studies have looked at deep learning methods specifically for malicious URL detection~\cite{le2018urlnet, Saxe2017, yu2020deephttp, yuan2018url2vec}. Le et al. design URLNet~\cite{le2018urlnet}, which uses Convolutional Neural Networks to generate a combined word and character vector representation, while Yu et al. design DeepHTTP~\cite{yu2020deephttp}, which uses  Bidirectional Long Short-Term Memory (Bi-LSTM) with attention mechanism to learn contextual relationships in HTTP traffic. 
%While URLNet and DeepHTTP build their own framework, another system called URL2Vec~\cite{yuan2018url2vec} leverages Word2Vec to learn character embeddings for detecting \emph{phishing} URLs. 




 \subsection{Overview}

\end{comment}

